Understanding Smart Contracts: Hype or Hope?

Smart Contracts are commonly considered to be an important component or even a key to many business solutions in an immense variety of sectors and promises to securely increase their individual efficiency in an ever more digitized environment. Introduced in the early 1990s, the technology has gained a lot of attention with its application to blockchain technology to an extent, that can be considered a veritable hype. Reflecting the growing institutional interest, this intertwined exploratory study between statistics, information technology, and law contrasts these idealistic stories with the data reality and provides a mandatory step of understanding the matter, before any further relevant applications are discussed as being "factually" able to replace traditional constructions. Besides fundamental flaws and applica-tion difficulties of currently employed Smart Contracts, the technological drive and enthusiasm backing it may however serve as a jump-off board for future developments thrusting well in the presently unshakeable traditional structures.

==> deprecated-tex/Data.tex <==
As in the work of \cite{oliva2020exploratory}, we cross-linked data from different sources. One of such sources is the \href{https://www.stateoftheDApps.com/}{``State of the DApps" (SDA)} \footnote{https://www.stateoftheDApps.com/} -- is a listing of decentralized Apps (DApps), where developers can list their DApps, additionally adding a category of the Dapp. Only the DApps stating the license as one of open source types were included into our research. One Dapp can consist of multiple SCs. To compare in this conventional software development, our Dapp is similar to a normal App and a SC can be seen as one coding script. As one App consists of multiple coding scripts, one Dapp consists of multiple interacting SCs. Using SDA's API in December, 2020 we obtained a list of all ETH Dapp that are listed there and hashaddresses of the SCs belonging to them. However, not all of them provide the information on the individual SCs belonging to them. \\

A second resource -- \href{https://etherscan.io/}{``Etherscan"} -- a platform that allows to monitor transactions, blocks and contracts on the ETH BC. Moreover, they offer the opportunity to verify the source code of a SC for informative purposes. Furthermore, their API provides with the opportunity to obtain the source code for such verified contracts. Therefore, using Etherscan we obtained the source codes for our DApps. To emphasize, not all DApps listed on SDA have verified contracts and not all DApps list their hashes. Therefore, the amount of possible codes is largely reduced. Moreover, Etherscan provides a list of last 10.000 verified contracts having open source licences. Therefore, we obtained a small labelled dataset with categories from SDA and larger unlabelled dataset. We highlight that only open source source codes obtained through Etherscan were obtained and moreover we do not intend to reuse or redistribute source code and thus  breach the copyright or code licences. \\

Moreover additional datasets, were obtained using BigQuery on \href{https://www.kaggle.com/}{``Kaggle}. By using BigQuery, we retrieved a list of all SC addresses on the ETH BC up to December, 2020. We created the following SQL query analogue to \cite{durieux2019empirical}. The exact query can be found in the Appendix.\\

The first dataset that we are going to use for classification contains of 1428 observations belonging to 473 distinct DApps. 20\% of observations were put aside as the test set. As we have a very small dataset, and some categories have very few observation, it was decided to summarize the categories except the first most-frequent 5 to the ``other" category. The second unlabelled dataset consists of 16250 SC's.

\begin{table}[H]
\begin{center}
 \begin{tabular}{lcc} 
 \hline
 \hline
 Topic & Amount of SCs &  Relative Amount of SCs \\ [0.5ex] 
 \hline
 Exchanges & 470 & 32.9\% \\ 
 Finance & 317 & 22.2\%  \\
 Games & 272 & 19.0\%  \\
 Gambling & 71 & 5.0\% \\
 High-risk & 60 & 4.2\% \\
 Marketplaces & 44 & 3.1\% \\
 Social & 41 & 2.9\%\\
 Media & 31 & 2.2\%\\
 Property & 29 & 2.0\%\\ 
 Development & 28  & 2.0\%\\ 
 Governance & 25 & 1.8\% \\
 Security & 13  & 0.9\%\\
 Identity & 12 & 0.8\%\\
 Wallet & 7 & 0.5\%\\ 
 Storage & 5 & 0.4 \% \\
 Health & 3 & 0.2\% \\ [1ex] 
 \hline
 All & 1428 & \\
 \hline
 \hline
\end{tabular}
\end{center}
    \vspace{-0.5cm}
 \caption{Categories in the Dataset 1
 \href{https://github.com/QuantLet/USC}{\includegraphics[keepaspectratio,width=0.4cm]{media/qletlogo_tr.png}}}\label{Tab:Categories}
\end{table}


==> deprecated-tex/Dataset_deprecated.tex <==
For this study we created a dataset using ETH historical data \textcolor{red}{consisting of XXX (update w/ JAN 2021 #)} available on Kaggle \citep{ethereum_kaggle}. By using BigQuery, we retrieved a list of all SC addresses and an individual list of corresponding transactions on the ETH BC up to March 10, 2020. We created the following SQL query analogue to \cite{durieux2019empirical}:\\

\begin{verbatim}
SELECT 
    contracts.address, COUNT(1) AS tx_count
FROM
    `bigquery-public-data.crypto_ethereum.contracts` AS contracts
JOIN
    `bigquery-public-data.crypto_ethereum.transactions` AS transactions
ON  (transactions.to_address = contracts.address)
GROUP BY contracts.address
ORDER BY tx_count DESC 
\end{verbatim}

\vspace{0.5cm}

Thus we were able to obtain \textcolor{red}{2 666 613} addresses. The majority - \textcolor{red}{1 096 965} contracts have only one corresponding transaction.  On a side-note, this means, that an immense amount of capital was used to either try out the functionalities, therefore also binding staff to do so, or other non-distillable reasons leading to \textcolor{red}{Kapital gebunden}.

For our analysis, we decided to take contracts having at least 100 transactions, this way we reduced the scope to \textcolor{red}{60 371} contracts.\\


Further data was obtained through different sources.
\href{https://www.stateofthedapps.com/}{``State of the DApps" (SDA)} -- is a listing of decentralized Apps (Dapps), where developers can list their Dapps, additionally adding a category of the Dapp. Using their API, we obtained a list of Dapps and the hashaddresses of the SCs belonging to them. A second resource -- ``Etherscan" -- a platform that allows to monitor transactions, blocks and contracts on the ETH BC. Moreover, they offer the opportunity to verify the source code of a SC for informative purposes. Furthermore, their API provides with the opportunity to obtain the source code for such verified contracts.\\


Thus, using the information from the SDA we obtained the source codes. Please note, for our analysis we used only the SCs that are under open-source licenses. If the type of license was not clear, we assumed the most strict type of license, therefore in ambiguous cases the source codes were not included in the research. The following categories were identified: 

\begin{table}[H] 
\centering
    \caption{Amount of SC in different categories} \label{datasets}
        \begin{tabular}{lcr}
                \hline
        \hline
        Category & \# of contracts & precentage \\ 
        \hline
        Exchanges   &    590  & 37.80\% \\
        Games       &    310  & 19.86\% \\
        Finance     &    278  & 17.80\% \\
        Gambling    &    69   & 04.42\% \\
        High-risk   &    57  & 03.65 \%  \\
        Social      &    45  & 02.88\% \\
        Marketplaces&     43 & 02.75\% \\
        Property    &     40 & 02.56\% \\
        Media       &    31  & 01.99\% \\
        Development &     29 & 01.86\% \\
        Governance  &     26 & 01.67\% \\
        Identity    &     12 & 00.77\% \\
        Security    &     12 & 00.77\% \\
        Wallet      &     10 & 00.64\% \\
        Storage     &      6 & 00.38\% \\
        Health      &      3 & 00.19\% \\
        \hline
        All         &    1561 \\
                \hline
        \hline
        \end{tabular}
\end{table}

Moreover, through the ``Etherscan" API we obtained source codes for \color{red}14 000 \color{black} open-source verified SCs source codes, not listed in SDA. Further supplementary research data was obtained from 
\href{www.hu.berlin/brc}{Blockchain-Research-Center.de \includegraphics[keepaspectratio,width=0.4cm]{CSC/media/BRC-klein_Bildmarke-Blau.jpg}}).

==> deprecated-tex/Methodology.tex <==
\subsection{SC Classification}
 In this section, we are going to propose using machine learning methods to as an approach to classify the category of SCs to have a tool that provides with the opportunity to further understand the ETH BC environment. Why using classification at all? As we could see in Figure \ref{Fig:SC_New_Total_Time}, the amount of transactions creating a SC on the ETH BC counts approximately 3.5 billions. On the other side, on the already mentioned Dapps listing website SDA, we can see the total amount of listed Dapps and the amount of the SCs these Dapps are consisting of. Currently there are around 3.5 thousands Dapps on the ETH BC and 6.49 thousand SCs. SO what are all these 99\% of the SCs lying on the BC. By training a classifier and achieving a good performance, we would gain a tool that could enable further exploration of the ETH SCs.

\subsubsection{Data Pre-processing and Feature Extraction} 
As mentioned in section \ref{DatasetSection}, we obtained a list of source codes. As a pre-processing step, we decided to use regular expressions to extract the comments from the source codes. Therefore, we created three columns: source code (full code), source code without comments (only code) and only comments (comments). Moreover, as additional feature engineering step, we extracted names of functions, contracts, events, interfaces and libraries and joined to one string. There exist different approaches to extract features from the source codes. Possible approaches are to extract features like names, design patterns or even abstract syntax trees. For our work, we decided to treat our code like text and to use similar technique to that used in natural language processing.

\subsubsection{Machine Learning methods}
To train our classificator, we decided to use the following methods: the most straight-forward approach -- a logistic regression, in our case we use a Ridge regression (Ridge) and also an instance of Lasso regression (Lasso). Since we have a very high-dimensional data, we expect the Lasso regression to perform better due to inherent feature selection technique through l1 regularization. Moreover, we are going to use random forest (RF) and support vector machines (SVM).\\
Depp learning methods are seen to be standard for natural language processing. However, they usually require huge datasets. Nonetheless, we would still try to apply three classical deep learning architectures: gated recurrent unit (GRU), bidirectional GRU, and convolutional neural network (CNN). All already mentioned methods will be applied on our small dataset on three different types of data: full code, only code, and comments. \\
Recently, pre-training become a standard for many natural language processing tasks. Bidirectional Encoder Representations from Transformers (BERT) architecture invented by \cite{devlin2018bert} allows the user to apply this deep learning architecture trained on a huge amount of data on a different task, e.g., text classification. These models achieve a state-of-the-art performance for many tasks. Moreover, they are able to work on relatively small datasets. Such architecture are usually pre-trained on huge text datasets. In our case, we have mostly the source codes, that differs from written and spoken human language, therefore it will not help us much. However, one of our tasks formulations includes machine learning on the comments. Therefore, we will be able to apply BERT on comments.\\
To summarize it, we are going to use traditional machine learning methods Ridge, Lasso, RF, and SVM and classical deep learning methods GRU, BGRU, and CNN on full code, only code, and comments. Moreover, we will apply BERT to the comments. Therefore, we will try to answer the question, whether it is possible at all to train a classifier on the solidity SC source code, whether traditional machine learning methods can better work on such small and high-dimensional dataset or they will loose to deep learning. Moreover, we will see whether it is better to train a classifier on the code, code with comments, or just comments, or even that, as opposed to spoken and written text, the sequential structure of the source code is not relevant at all to identify the category of the SC. 

\subsubsection{Training and Evaluation}
For training we used cross-validation approach with 3 folds. Moreover, we performed a hybrid of manual and automatic grid hyper-parameter tuning. As we are dealing with a multiclass classification task  with one class containing examples from the rest of categories, we decided to use the one-vs-all classification approach for the first 5 classes. For the evaluation we used two metrics: Area under the ROC curve is equivalent to ``the probability that the classifier will rank a randomly chosen positive instance higher than a randomly chosen negative instance" \citep{fawcett2006introduction} and the average precision -- the metric which is seen as standard for unbalanced data sets.

\subsection{Clustering}
In the \ref{Literature_Review} section we already applied clustering on the Scopus dataset to identify the trending groups. This strategy will be also applied to a bigger unlabelled dataset to try to identify possible groups, using the comments in the SCs. Originally, the approach was inspired by the blogpost ``Topic Modeling with BERT" \citep{topic2020}.
As we are dealing with a very high-dimensional dataset, the first step is to reduce the dimensionality of the data. For this purpose we use the uniform manifold approximation and projection for dimension reduction (UMAP) technique, recently proposed by \cite{mcinnes2018umap}, which already gained a lot of popularity due to its fast computations and ability to preserve global structure. First, we encoded our data using already mentioned BERT, it is possible to load only the embeddings -- the lower dimensional representation of words. Even though these embeddings are of lower dimension than the original data, it is still has too many dimensions to perform clustering. Many clustering methods are based on distances and the more dimensions data has, the more options arise to separate such data. Thus using UMAP, we reduced our dataset to 5 dimensions and in the case of literature research example, we used K-means clustering methods to identify 14 topics. How we decided on the number 14 was already described in \ref{Literature_Review}. Followingly, we applied UMAP again to obtain 2 dimensions to be able to plot our  data points. In the blogpost, \cite{topic2020} proposes a variant of TF-IDF -- the class-based variant of TF-IDF (c-TF-IDF), whcih author formulates as the following: 

\begin{equation*}
    c-TF-IDF_i = \frac{t_i}{w_i}  \times \log \frac{m}{\sum^n_jt_j},
\end{equation*}

where $t$ is the frequency of each word, $i$ -- the class i, $w$ is the total number of words for i-th class, $m$ is the number of documents, and $\sum^n_jt_j$ -- the total frequency of word $t$ across all classes $n$. For each category, in our case topic, we identified the top ten of the msot important words. Similar approach was used to group unlabelled SCs using their comments.

==> deprecated-tex/Methodology_deprecated.tex <==


DESCRIBE THE FOLLOWING ESSENTIAL PAPERS - UP TO LITERATURE REVIEW ASWELL!!!



\begin{itemize}
    \item \url{https://arxiv.org/pdf/1702.05511.pdf}
    \item \url{https://arxiv.org/pdf/1703.06322.pdf}
    \item \url{https://eprints.cs.univie.ac.at/5665/1/bare_conf.pdf}
    \item \url{https://arxiv.org/pdf/1911.00169.pdf}
    \item \url{https://link.springer.com/article/10.1007/s10664-019-09796-5} IMPORTANT
    \item \url{https://www.ccs.neu.edu/home/amislove/publications/Ethereum-IMC.pdf}
\end{itemize}














%%%%%%%%%%%%NEXT%%%%%%%%%%%%%%






 
 
 
 \newpage
 
 








%%%%%%%%%%%%NEXT%%%%%%%%%%%%%%
 
 
 







\subsection{Classification Methodology}
In this section, we are going to describe the methodology we use in our research to classify and cluster our SCs.

ALGO's

\begin{itemize}
    \item \url{https://orbilu.uni.lu/bitstream/10993/36755/1/automated-labeling-unknown.pdf}
    \item \url{https://eprints.cs.univie.ac.at/5433/7/sanerws18iwbosemain-id1-p-380f58e-35576-preprint.pdf}
    \item \url{https://ieeexplore.ieee.org/stamp/stamp.jsp?arnumber=9019682&tag=1} (IMPORTANT DL)
    \item \url{https://arxiv.org/pdf/1802.01517.pdf}
    \item \url{https://onlinelibrary.wiley.com/doi/full/10.1002/smr.2267}
    \item \url{https://link.springer.com/article/10.1007/s10664-020-09852-5}
    \item \url{https://arxiv.org/pdf/2001.07125.pdf}
\end{itemize}





%%%%%%%%%%%%NEXT%%%%%%%%%%%%%%






 
 
 
 \newpage
 
 








%%%%%%%%%%%%NEXT%%%%%%%%%%%%%%
 





\subsection{Source Code Review and Empirical Taxonomy}
\label{SourceCode}


%  \textcolor{red}{Electronic Signatures}\\
 
%   \textcolor{red}{https://medium.com/mycrypto/the-ethereum-virtual-machine-how-does-it-work-9abac2b7c9e}\\

%   \textcolor{red}{https://yos.io/2019/04/14/erc-standards-you-should-know-about/
% }\\


Unlike traditonal contracts, SC's are not written in natural language, which makes it hard to determine what each contract is about. This was our motivation to start working towards a predictive model that would classify smart contracts, based solely on their codes. Our work, so far, has been focused on going through the source code of 800 certified smart contracts, provided by \cite{etherscan}, and manually labeling them into 9 different categories. The categories that we came up with are:

\begin{itemize}
	\item \textbf{Token creation}, \textbf{Token sale} or \textbf{Token creation/Token sale}: when contract's sole purpose is to define a token, or its crowdsale, or both.
\vspace{-0.3cm}
	\item \textbf{Finance} or \textbf{Token creation/Finance}: whenever a contract has an implementation of a financial product or a derivative, a bidding mechanism, a lottery, a multisignature wallet, or in general any profit-creating mechanism. A token can be implemented in a separate contract and be evoked, or defined in a Finance contract directly. 
\vspace{-0.3cm}
	\item \textbf{Airdrop} or \textbf{Token creation/Airdrop}: an implementation of a token airdrop, sometimes simultaneously with a token definition. An airdrop is a free distribution of a token, unlike a crowdsale.
\vspace{-0.3cm}
	\item \textbf{DApp}: an implementation of an Ethereum DApp.
\vspace{-0.3cm}
	\item \textbf{Scam}: pyramid schemes, or financial contracts that offer e.g. 5 percent daily interest.
\vspace{-0.3cm}
	\item \textbf{Utility}: diverse helper functions, pieces of code that are necessary for running actual contracts, extensions, libraries, etc.
\end{itemize}

Next we discuss technical characteristics of the SC's that we went through, the challenges that arise when it comes to implementing them in current systems, as well as the main drawbacks of the current coding practices and how they can be improved.







%%%%%%%%%%%%NEXT%%%%%%%%%%%%%%






 
 
 
 \newpage
 
 








%%%%%%%%%%%%NEXT%%%%%%%%%%%%%%
 




\subsection{Pre-processing and Feature Engineering}

\subsection{Classification, Clustering, and Evaluation}



\begin{itemize}
    \item TML vs DL
    \item can DL help, when we have such small data
    \item do we need the source code, or only identifiers (function, contract names, etc) --> THIS IS DIFFERENT TO OTHER LANGUAGES PARADIGMS THAN SOLIDITY
\end{itemize}


In the previous section, we showed the potential of the supervised classification. Like in many machine learning domains, obtaining labeled data can be not only difficult and costly, but also it can introduce a selection bias. In our case, having the data which is listed by the developers, we only obtain the categories where developers are interested to disclose the information. However, all those that are interested to be undisclosed are not taken into account. Thus, in this section, we would like to identify the optimal amount of clusters of our dataset. In \ref{Fig:elbow}, the reader can find the elbow-curve: a methodology to find the optimal $k$ for the K-Means clustering approach. On the x-axis the $k$ parameter is depicted, whereas on the y-axis, we can find the distortion -- sum of squared distances of samples to their closest cluster center. \\




\begin{figure}[H]
	\centering
	\includegraphics[keepaspectratio,width=17cm]{elbow.png}
        \caption{***Elbow Curve}
		\href{https://github.com/QuantLet/CSC_Dapps}{\includegraphics[keepaspectratio,width=0.4cm]{media/qletlogo_tr.png}}
        \label{Fig:elbow}
\end{figure}



We observe multiple ``elbows": 3, 5, 14, 16, 17. Interestingly, the first elbow of 3 could correspond to the three biggest labelled categories. Whereas 17 correspond to the true amount. In \ref{Fig:cl3}, data is depicted categorized to 3 categories, whereas in \ref{Fig:labels} the original self-reported categories are pictured. Comparing both figures, we can conclude that the identified clusters do not necessarily correspond to the true categories.\\

\color{red}{REMOVE LEGEND + REARRANGE PARALLEL + ADD FOR OTHER k}



\begin{figure}[H]
	\centering
	\includegraphics[keepaspectratio,width=17cm]{images/tsne_clustering_3.png}
        \caption{Clustering k=3, 20150630-20201001}
		\href{https://github.com/QuantLet/CSC_Dapps}{\includegraphics[keepaspectratio,width=0.4cm]{media/qletlogo_tr.png}}
        \label{Fig:cl3}
\end{figure}




\begin{figure}[H]
	\centering
	\includegraphics[keepaspectratio,width=17cm]{images/tsne_llabels_3.png}
        \caption{Labels, 20150630-20201001}
		\href{https://github.com/QuantLet/CSC_Dapps}{\includegraphics[keepaspectratio,width=0.4cm]{media/qletlogo_tr.png}}
        \label{Fig:labels}
\end{figure}








\color{red}{DO WE IDENTIFY ALL GROUPS? OR CAN WE MATHEMATICALLY SEE MORE? \\
DO THE CLUSTERS GROUPS CORRESPOND TO THE LABELS? \\
ELBOW CURVE FOR CLUSTERING -> OPTIMAL AMOUNT OF CLUSTERS}\\




\color{black}












%%%%%%%%%%%%NEXT%%%%%%%%%%%%%%






 
 
 
 \newpage
 
 








==> deprecated-tex/Results.tex <==
In this section, we are going to describe the results of classification which methodology was just presented. In the following tables, we present the results of our classification training in terms of AUC ROC and average precision (Av. Prec.) for the test data. Due to spatial reasons we present only the test performance, nonetheless, cross-validation performance can also be found on GitHub in the respective Jupyter Notebooks. In Table \ref{Tab:results_FC}, we see the results of classificator trained on the full code -- without removal of comments. On the left part we see the performance in terms of AUC ROC, which is relatively high for all categories. Methods of traditional machine learning methods outperform on average the methods of deep learning. One of the possible and very probable reasons is the small amount of data points, whereas the big size of a dataset is essential for application of deep learning methods. On the other side, as opposed to our expectation Lasso regression showed the worst performance across all traditional machine learning methods. Random forest shows the best performance in terms of AUC ROC in almost all categories, except high risk, where it is outperformed by the Ridge regression. Ridge shows the second best performance in all other categories. On the right part, we see the performance in terms of Av. Prec. Whereas the performance for classes with a higher amount of examples is still high, the classes that are outnumbered show much lower performance. Gambling and High-risk classes show the worst ability to be accurately classified. Moreover, deep learning methods show a very poor performance for such unbalanced categories. In table \ref{Tab:results_OC}, we see the performance of the classificators trained on the code cleaned from the comments. It shows very similar tendency: a good performance of rather simple traditional machine learning methods like RF and Ridge and very poor performance of neural networks. Interestingly, there is no obvious tendency of outperforming between results on the source code with and without comments. In the next Table \ref{Tab:results_comments}, we present results of predictors trained only on textual data -- the comments extracted from the code. Again, traditional methods outperform deep neural networks. Some categories, such as Exchanges, show even better performance than classificators  trained on code. A possible explanation could be the quality of the comments in the codes of this category. However, other groups show worse performance, except Gambling in terms of Av. Prec. Apparently, the comments allow the ridge regression to correctly pick the Gambling cases with higher precision and judging by lower AUC ROC, the False Positives rate increased. Interestingly, even BERT that is seen as a deep learning model that is able to deal with small datasets shows a very poor performance. \\

As we were able to show that deep learning networks, especially those based on recurrence and reflecting the sequential structure, show poor performance, it would be interesting to inspect, whether we are able to extract the most important features from the code. As explained in the \ref{Methodology} part, we decided to extract the names of functions, events, libraries in the hope that they can be not only similar from the source code to source code, since as already mentioned many codes are cloned and copied, but also usually developers would name the variables and functions according to their behavior. In table \ref{Tab:results_features}, we show the results of classification training of traditional machine learning methods, which have shown the best performance in the previous tasks. The aim was to show that not only can we extract meaningful information and the sequential structure is not important for our task but also that we are able to achieve sufficiently high performance using lower amount of features. And as we see in this table, we still have high performance, even though the amount of features was reduced by more than 3 thousands. \\

Therefore, with this section we were able to show that it is possible to classify the SCs using their source codes quite accurately for at least 4 categories: Exchange, Finance, Games, High-Risk. Such information can be useful not only for researcher who want to explore the rest 99\% of SC on the ETH BC, but also for the developers and investors. Especially the high-risk category is interesting in identification of possible risks.

\begin{table}[H]
    \begin{center}
        {\scriptsize
        \scalebox{0.9}{
        \begin{tabular}{lcccccccccc}
        \hline 
        \hline
              \toprule
            Method &
            \multicolumn{5}{c}{AUC ROC} &
            \multicolumn{5}{c}{Av.Prec}\\ 
             & {Exchanges} & {Finance} & {Gambling} & {Games} & {High-risk} & {Exchanges} & {Finance} & {Gambling} & {Games} & {High-risk} \\ 
             \hline
             Ridge & 0.988 & 0.967 & 0.914 & 0.972 & 0.983 & 0.985 & 0.925 & 0.482 & 0.914 & 0.720 \\
             Lasso & 0.961 & 0.927 & 0.714 & 0.917 & 0.847 & 0.962 & 0.844 &	0.238 &	0.804 &	0.554\\
             RF & 0.988 & 0.973 & 0.944 & 0.971 & 0.974 & 0.984 & 0.942 & 0.572 &	0.912 &	0.700 \\
             SVM & 0.987 &	0.972 &	0.892 &	0.977 &	0.976 &	0.983 &	0.944 &	0.482 &	0.934 &	0.668  \\ 
             BGRU & 0.970 &	0.848 &	0.767 &	0.795 &	0.860 &	0.963 &	0.699 &	0.149 &	0.422 &	0.256	\\ 
             GRU & 0.966 &	0.712 &	0.749 &	0.818 &	0.897 &	0.956 &	0.443 &	0.102 &	0.442 &	0.486 \\ 
             CNN & 0.972 &	0.950 &	0.804 &	0.908 &	0.840 &	0.972 &	0.880 &	0.155 &	0.672 &	0.482\\
        \hline
        \hline
        \end{tabular}}
        }
    \end{center}
    \vspace{-0.5cm}
        \caption{Classification Results -- Full Code
        \href{https://github.com/QuantLet/USC}{\includegraphics[keepaspectratio,width=0.4cm]{media/qletlogo_tr.png}}}  \label{Tab:results_FC}
\end{table} 




\begin{table}[H]
    \begin{center}
        {\scriptsize
        \scalebox{0.9}{
        \begin{tabular}{lcccccccccc}
        \hline 
        \hline
              \toprule
            Method &
            \multicolumn{5}{c}{AUC ROC} &
            \multicolumn{5}{c}{Av.Prec}\\ 
             & {Exchanges} & {Finance} & {Gambling} & {Games} & {High-risk} & {Exchanges} & {Finance} & {Gambling} & {Games} & {High-risk} \\ 
             \hline
             Ridge & 0.983 & 0.965 & 0.916 &	0.957 &	0.988 &	0.981 &	0.914 & 0.483 & 0.868 & 0.795 \\
             Lasso & 0.960 & 0.915 & 0.832 &	0.922 &	0.934 &	0.959 &	0.813 & 0.363 & 0.769 & 0.656\\
             RF & 0.986 & 0.974 & 0.938 &	0.966 &	0.986 &	0.983 &	0.940 &	0.491 &	0.907 &	0.771 \\
             SVM & 0.980 & 0.973 & 0.905 &	0.970 &	0.976 &	0.979 &	0.943 &	0.574 &	0.919 &	0.717 \\ 
             BGRU & 0.946 &	0.282 &	0.461 &	0.744 &	0.763 &	0.952 &	0.157 &	0.049 &	0.448 &	0.508	\\ 
             GRU & 0.949 &	0.802 &	0.779 &	0.692 &	0.888 &	0.952 &	0.615 &	0.121 &	0.299 &	0.350 \\ 
             CNN & 0.952 & 0.895 &	0.707 &	0.868 &	0.781 &	0.953 &	0.794 &	0.100 & 0.663 &	0.168\\
        \hline  
        \hline
        \end{tabular}}
        }
    \end{center}
    \vspace{-0.5cm}
    \caption{Classification Results -- Only Code
    \href{https://github.com/QuantLet/USC}{\includegraphics[keepaspectratio,width=0.4cm]{media/qletlogo_tr.png}}}\label{Tab:results_OC}
\end{table} 


\begin{table}[H]
    \begin{center}
        {\scriptsize
        \scalebox{0.9}{
        \begin{tabular}{lcccccccccc}
        \hline 
        \hline
              \toprule
            Method &
            \multicolumn{5}{c}{AUC ROC} &
            \multicolumn{5}{c}{Av.Prec}\\ 
             & {Exchanges} & {Finance} & {Gambling} & {Games} & {High-risk} & {Exchanges} & {Finance} & {Gambling} & {Games} & {High-risk} \\ 
             \hline
             Ridge & 0.991 & 0.959 & 0.88 &	0.972 & 0.976 &	0.986 &	0.910 &	0.508 &	0.912 &	0.701 \\
             Lasso & 0.982 & 0.930 &	0.734 &	0.942 &	0.880 &	0.977 &	0.852 &	0.217 &	0.844 &	0.409\\
             RF & 0.984 & 0.972	& 0.890 & 	0.974 &	0.977 &	0.981 &	0.937 &	0.452 &	0.924 &	0.675 \\
             SVM & 0.988 &	0.963 &	0.879 &	0.978 &	0.976 &	0.983 &	0.921 &	0.511 &	0.933 &	0.626 \\ 
             BGRU & 0.971 &	0.639 &	0.656 &	0.853 &	0.839 &	0.968 &	0.276 &	0.086 &	0.520 &	0.361	\\ 
             GRU & 0.960 & 0.804 & 0.638 &	0.840 &	0.855 &	0.963 &	0.648 &	0.107 & 0.511 &	0.313 \\ 
             CNN & 0.937 &	0.907 &	0.829 &	0.865 &	0.703 &	0.937 &	0.799 &	0.155 &	0.600 &	0.070\\
             BERT & 0.968 &	0.777 &	0.353 &	0.789 &	0.602 &	0.965 &	0.637 &	0.038 &	0.628 &	0.056\\
        \hline  
        \hline
        \end{tabular}}
        }
    \end{center}
    \vspace{-0.5cm}
    \caption{Classification Results -- Only Comments
    \href{https://github.com/QuantLet/USC}{\includegraphics[keepaspectratio,width=0.4cm]{media/qletlogo_tr.png}}}
    \label{Tab:results_comments}
\end{table} 

\begin{table}[H]
    \begin{center}
        {\scriptsize
        \scalebox{0.9}{
        \begin{tabular}{lcccccccccc}
        \hline 
        \hline
              \toprule
            Method &
            \multicolumn{5}{c}{AUC ROC} &
            \multicolumn{5}{c}{Av.Prec}\\ 
             & {Exchanges} & {Finance} & {Gambling} & {Games} & {High-risk} & {Exchanges} & {Finance} & {Gambling} & {Games} & {High-risk} \\ 
             \hline
             Ridge & 0.988 & 0.963 &	0.883 &	0.957 &	0.971 &	0.984 &	0.906 &	0.462 &	0.870 &	0.735 \\
             Lasso & 0.981 & 0.919 &	0.803 &	0.913 &	0.874 &	0.973 &	0.791 &	0.395 &	0.730 &	0.573 \\
             RF & 0.989	& 0.971 & 0.864 &	0.961 &	0.973 &	0.985 &	0.928 &	0.474 &	0.899 &	0.719\\
             SVM & 0.980 & 0.963 & 0.877 &	0.971 &	0.970 &	0.978 &	0.932 &	0.489 &	0.915 &	0.754 \\ 
        \hline   
        \hline
        \end{tabular}}
        }
    \end{center}
    \vspace{-0.5cm}
    \caption{Classification Results -- Extracted Features
    \href{https://github.com/QuantLet/USC}{\includegraphics[keepaspectratio,width=0.4cm]{media/qletlogo_tr.png}}}
    \label{Tab:results_features}
\end{table} 

==> deprecated-tex/literature_review.tex <==
Existing research on SC's is very diverse. Researchers focus on variety of aspects, ranging from applications of SC's in healthcare and quality monitoring \citep[e.g.,][]{Celesti2020, Khatoon2020, Yu202012479}, technical implementations and vulnerabilities \citep[e.g.,][]{Ajienka2020, Pierro20201, Li2020438} to games \citep[e.g.,][]{scholten2019ethereum}. Our research is mostly related to the empirical analysis of the ETH blockchain itself, statistics and categorization of its usage and possibilities that ETH brings with itself. \\

One of the first research works dedicated to the empirical analysis of SCs is the work by \cite{bartoletti2017empirical}. The authors gathered a dataset of 834 SC source codes, which were then manually classified into different categories using the proposed taxonomy. The identified categories contained types like Notary, Financial, Game, Wallet, Library. Moreover, authors were able to identify the design pattern found in the source code. This work is not the only one approaching the SC topic from the software engineering perspective as of any other technology using programming languages. \cite{wohrer2018design} also dedicate their work to design patterns that are aimed to improve and facilitate the work of software developers and engineers working on applications for the blockchain, as similar problems may require similar solutions. One of the later empirical studies created by \cite{oliva2020exploratory} propose the approach of cross-linking the data from different sources in order to better scrutinize their behavior: their activity level, category of what these contracts are and source code metrics, like complexity. Our work is inspired to a big extent by the work of \cite{oliva2020exploratory}, nonetheless we are aiming to extend it with legal perspective and a proposal of approaches to gain opportunities for further ETH exploration. \\

Other relevant for our paper research direction is the automatic source code classification. To emphasize the importance of automatic categorization, we repeat that some of the previous work is done manually, such as \cite{bartoletti2017empirical}. Although the idea of using machine learning for code classification is not very new, it is not that present in the ETH realm, as we will see the evidence for it later in this section. However, such research exists. \cite{norvill2017automated} use unsupervised techniques and run clustering on bytecodes to group contracts with similar purpose. Not only unsupervised techniques can be used to identify different structures in the smart contracts. \cite{chen2018detecting} use machine learning method XGBoost on the opcodes and account data to identify Ponzi schemes. \cite{wang2020contractward} use different machine learning methods to identify security vulnerabilities in SCs. Many codes on the ETH blockchain are very similar and quite often can be copied. \cite{kondo2020code} investigate code cloning on ETH and  identify clusters of the code clones and inspect their behavior.
Our aim is not only to show the directions that are most relevant for our further analysis, but also to present a holistic view on the concept of SCs, including the research. Therefore we are going to summarize the research as a global picture. \\

For this purpose we utilized \href{https://www.scopus.com/home.uri}{Scopus citation and abstract database}\footnote{https://www.scopus.com/home.uri} that gathers peer-reviewed research from around 11.7 thousand publishers from different directions in science. The query retrieves the scholarly work from conferences and journals in English language containing ``ethereum" or ``smart contracts" in the title. Furthermore, the query limited to work conducted in the areas like Business, Computer and Decision science and Mathematics. The exact query can be found in the Appendix. Thus, we obtained a list 839 research outlets. As observable in figure \ref{fig:Research-years}, research publishing on ETH SC's began in 2016 -- which is to predictable since the ETH BC was introduced in July 2015. Thereafter, the amount of research started to increase and achieved a peak in 2019. At the date of retrieving the query, the year 2020 was ongoing, hence we cannot fully measure whether the amount of research in 2020 is higher or lower compared to 2019. Nonetheless, we can see that the interest in the SC area is not fading and is staying on a quite high level. \\

The topics of the examined research outputs were distilled from their individual abstracts and keywords. We present the most frequent keywords as a wordcloud in Figure \ref{fig:wordcloud}. The keywords ``blockchain", ``smart contract", and ``ethereum" were filtered out since they were used to limit the query due to absence of additional semantic information. Technical keywords keywords such as ``security", ``data", ``iot", ``solidity", ``distributed ledger", and ``decentralized" are the most frequently used. Unfortunately, these do not provide us with sufficient additional information to identify clear tendencies in the research and hence each of these keywords could belong to any given paper in the field of SC research.\\

To scrutinize our data further, we decided to group our research papers into topics they are dedicated to, using dimensionality reduction, clustering and natural language processing techniques and, subsequently, inspect the most important words used in research papers in the respective topic. This analysis was performed on the abstract and not on the keyword level, to achieve higher specification. Due to the fact that we utilize this technique twice in our research, the technical implementation in a greater detail is described in the section \ref{sec:Methodology}. The only technical detail that is necessary to mention here is the approach of how to identify the optimal amount of groups/clusters. We utilized the elbow curve method - a heuristic to identify the number of clusters in a dataset, which origin is sometimes traced to \cite{thorndike1953belongs}. The main idea of this elbow curve method is to measure the identified performance metric for different numbers of groups, plot them against each other and identify points that are knee or elbow of the curve. Mathematically it can be formulated in terms of the second derivative. The possible metrics for clustering could be an intra- or intercluster variance. The Silhouette score \citep{rousseeuw1987silhouettes} - the measure of how an object is similar to its own cluster and Davies-Bouldin score \citep{davies1979cluster} - the average similarity measure of each cluster with its most similar cluster were used in our case, which is depicted in Figure \ref{fig:Elbow_curves_literature}.

\begin{figure}[H]
\centering
\hfill
\subfigure[Amount of research on SC issued within last years]{\includegraphics[width=7cm]{CSC/images/year_frequency.png}\label{fig:Research-years}}
\hfill
\subfigure[Wordcloud of existing research keywords]{\includegraphics[width=7cm]{CSC/images/wordcloud.png}\label{fig:wordcloud}}
\hfill
\caption{Existing research \href{https://github.com/QuantLet/CCID/tree/master/CCIDvolumeGAM}{\includegraphics[keepaspectratio,width=0.4cm]{media/qletlogo_tr.png}}}
\label{fig:research}
\end{figure}

\begin{figure}[H]
\centering
\hfill
\subfigure[Silhouette score]{\includegraphics[width=7cm]{CSC/images/silhouette.png}\label{fig:Silhouette}}
\hfill
\subfigure[Davies-Bouldin score]{\includegraphics[width=7cm]{CSC/images/davies.png}\label{fig:Davies}}
\hfill
\caption{Identification of optimal number of groups \href{https://github.com/QuantLet/CCID/tree/master/CCIDvolumeGAM}{\includegraphics[keepaspectratio,width=0.4cm]{media/qletlogo_tr.png}}}
\label{fig:Elbow_curves_literature}
\end{figure}

Judging the optimal amount of groups using these figures was not unambiguous in our case. Multiple values could be seen as ``elbows". We decided to have a granular clustering, therefore the highest number within the possible ``elbows" was taken, which is 14. After grouping the existing research into 14 different groups, we identified the top ten of the most ``important" words of each topic to gather a feeling on what these topics can be dedicated to. Through manual subjective assessment, the following categories were identified:  \textcolor[HTML]{286896}{Blockchain general}, \textcolor[HTML]{de762b}{bitcoin/cryptocurrency research}, \textcolor[HTML]{338734}{Voting/payment}, \textcolor[HTML]{b93638}{Authorization/access}, \textcolor[HTML]{8766a8}{Ponzi/vulnerabilities (non-technical)}, \textcolor[HTML]{79514a}{Manufacturing},\textcolor[HTML]{d179b4}{Oracle/cloud},\textcolor[HTML]{6a6a6a}{Agriculture/food},
\textcolor[HTML]{9fa132}{Mining/validating}, \textcolor[HTML]{23a1af}{SC research papers}, \textcolor[HTML]{0a1064}{Healthcare/medical}, \textcolor[HTML]{7c39c3}{Attacks/vulnerabilities (technical)}, \textcolor[HTML]{e78379}{Auction/bidding}, \textcolor[HTML]{429a68}{Energy prosumer}. The colors correspond to the colors in Figures \ref{fig:topics_research_1} and \ref{fig:topics_research_2}. In the following Figure \ref{fig:Literature_scatter}, we can see the scatter plot, depicting our clustering into different topics of the existing research. Not only can we see that the topics are very versatile, but also that they are inter-related and some are more distant from other topics than others. Furthermore, we can also conclude that there are no such topics that would dominate bigger parts of the research. Nonetheless, we can see that the biggest clusters are dedicated to the general \textcolor[HTML]{de762b}{bitcoin/cryptocurrency research} and to the \textcolor[HTML]{338734}{Voting and payment} technologies using SC on blockchain. Rather smaller clusters are dedicated to problems like \textcolor[HTML]{0a1064}{Healthcare/medical}, \textcolor[HTML]{6a6a6a}{Agriculture/food} and general metaresearch on \textcolor[HTML]{23a1af}{SC research}. Going back to the first part of this section, we would like to emphasize the fact that there are no clusters containing distinctly related machine learning key-words. Therefore, we were able to show that research on SC covers multiple directions and there are no tendencies that would obviously dominate the research. How representative it is for the real-world use-cases we would try to show in the later sections. Moreover, the fact of essentially discipline-capsuled and non-intertwined research can be also deduced from our analysis.


\begin{figure}[H]
\hfill
\subfigure[Topic 1]{\includegraphics[width=5.3cm]{CSC/images/topics/Topic_0.png}}
\hfill
\subfigure[Topic 2]{\includegraphics[width=5cm]{CSC/images/topics/Topic_1.png}}
\hfill
\subfigure[Topic 3]{\includegraphics[width=4.9cm]{CSC/images/topics/Topic_2.png}}
\hfill
\subfigure[Topic 4]{\includegraphics[width=5.5cm]{CSC/images/topics/Topic_3.png}}
\hfill
\subfigure[Topic 5]{\includegraphics[width=4.9cm]{CSC/images/topics/Topic_4.png}}
\hfill
\subfigure[Topic 6]{\includegraphics[width=5cm]{CSC/images/topics/Topic_5.png}}
\hfill
\subfigure[Topic 7]{\includegraphics[width=5.4cm]{CSC/images/topics/Topic_6.png}}
\hfill
\subfigure[Topic 8]{\includegraphics[width=5cm]{CSC/images/topics/Topic_7.png}}
\hfill
\subfigure[Topic 9]{\includegraphics[width=4.7cm]{CSC/images/topics/Topic_8.png}}
\hfill
\caption{Top 10 the most important words per topic identified in the existing SC research (Part 1) \href{https://github.com/QuantLet/CCID/tree/master/CCIDvolumeGAM}{\includegraphics[keepaspectratio,width=0.4cm]{media/qletlogo_tr.png}}}
\label{fig:topics_research_1}
\end{figure}

\begin{figure}[H]
\hfill
\subfigure[Topic 10]{\includegraphics[width=5.4cm]{CSC/images/topics/Topic_9.png}}
\hfill
\subfigure[Topic 11]{\includegraphics[width=4.8cm]{CSC/images/topics/Topic_10.png}}
\hfill
\subfigure[Topic 12]{\includegraphics[width=5.1cm]{CSC/images/topics/Topic_11.png}}
\hfill
\subfigure[Topic 13]{\includegraphics[width=5.5cm]{CSC/images/topics/Topic_12.png}}
\hfill
\subfigure[Topic 14]{\includegraphics[width=5.2cm]{CSC/images/topics/Topic_13.png}}
\hfill
\includegraphics[width=4cm]{CSC/images/topics/empty.png}
\hfill
\caption{Top 10 the most important words per topic identified in the existing SC research (Part 2) \href{https://github.com/QuantLet/CCID/tree/master/CCIDvolumeGAM}{\includegraphics[keepaspectratio,width=0.4cm]{media/qletlogo_tr.png}}}
\label{fig:topics_research_2}
\end{figure}


\begin{figure}[H]
\centering
\includegraphics[width=17cm]{CSC/images/scatter_research.png}
\caption{Grouping the existing research into 14 topics \href{https://github.com/QuantLet/CCID/tree/master/CCIDvolumeGAM}{\includegraphics[keepaspectratio,width=0.4cm]{media/qletlogo_tr.png}}}
\end{figure}\label{fig:Literature_scatter}




==> deprecated-tex/literature_review_deprecated.tex <==
The empirical analysis of SC's is a new research domain that is effectively lacking on interdisciplinary outlets. Current research offers no common ground understanding of the herewithin shown taxonomy of: 
\begin{itemize}
	\item FinTech-driven BC-based SC constructions structures and their modi that are inseparable meshed with the financial system and the conditioning legal framework.
   \vspace{-0.3cm}
	\item the corresponding challenges these proposed systemically disruptive problem-solving and process-optimizing approaches pose to the efficacy of the individual applicant and to their regulatory framework.
   \vspace{-0.3cm}
	\item the basic objective critical questioning and soundness of emphasizing the implementation of such technology into $any$ given kind of structure.
\end{itemize}

%\vspace{0.3cm}
To summarize and categorize the existing research - instead of pointing out a short list of handpicked examples to underline our arguments - we utilized the \href{https://www.scopus.com/home.uri}{Scopus citation database} limiting our search to journal and conference works given in English on \href{https://ethereum.org/en/}{Ethereum} (we will use the abbreviation ``ETH" for this system, while being fully aware of the respective ticker symbol - see further section \ref{Sec:FrameworkInfo}). We thus obtained a bias-free list of 839 research outlets and identified trends SC research, which are underlining the fact of essentially discipline-capsuled and non-intertwined research.


%Moreover, the limitation was set to the domains of Computer Science, Engineering, Decision.\\


\begin{figure}[H]
	\centering
	\includegraphics[keepaspectratio,width=13cm]{year_frequency.png}
        \caption{SC Research Output}
		\href{https://github.com/QuantLet/CSC_Dapps}{\includegraphics[keepaspectratio,width=0.4cm]{media/qletlogo_tr.png}}
        \label{Fig:dist}
\end{figure}






As observable in figure \ref{Fig:dist}, research publishing on ETH SC's began in 2016 - which is to predictable since the ETH BC was introduced in July 2015. Thereafter, the amount of research started to increase and achieved a peak in 2019. At the date of writing this, the year 2020 is ongoing, hence we cannot fully measure whether the amount of research in 2020 is higher or lower compared to 2019.\\

The topics of the examined research outputs were distilled from their individual abstracts and keywords. We present the most frequent keywords as a wordcloud in figure \ref{Fig:wordcloud}. The keywords and ``blockchain", ``smart contract", and ``ethereum" were filtered since they were used to limit the query due to absence of additional semantic information.




\begin{figure}[H]
	\centering
	\includegraphics[keepaspectratio,width=16cm]{wordcloud.png}
        \caption{Popular SC Keywords}
		\href{https://github.com/QuantLet/CSC_Dapps}{\includegraphics[keepaspectratio,width=0.4cm]{media/qletlogo_tr.png}}
        \label{Fig:wordcloud}
\end{figure}


Technical keywords keywords such as ``security", ``data", ``iot", ``solidity", ``distributed ledger", and ``decentralized" are the most frequently used. Unfortunately, these do not provide us with sufficient additional information to identify clear tendencies and hence each of these keywords could belong to any given paper in the field of SC research.\\
Therefore, we would like to identify clusters of research papers within extant research. For this purpose, we used the above described Scopus dataset. \color{orange} In order to extract a more detailed description of topics, we decided to use the whole abstracts and not only the keywords. \color{black} First, we applied the UMAP \color{orange} [CITE] \color{black} technique in order to reduce the dimensionality of the abstracts. We reduced our data into 5 dimensions. Subsequently, the K-Means clustering was applied on the dataset. To identify the optimal amount of clusters the elbow curve methodology was used. Using different metrics, Silhouette and Davis-Bouldin Score


\begin{figure}[H]
\centering
\includegraphics[width=13cm]{silhouette.png}
\href{https://github.com/QuantLet/CSC_Dapps}{\includegraphics[keepaspectratio,width=0.4cm]{media/qletlogo_tr.png}}
\caption{Determining the optimal number of clusters with Silhouette coefficient}
\label{fig:Silhouette}
\end{figure}

\begin{figure}[H]
\centering
\includegraphics[width=13cm]{davies.png}
\href{https://github.com/QuantLet/CSC_Dapps}{\includegraphics[keepaspectratio,width=0.4cm]{media/qletlogo_tr.png}}
\caption{Determining the optimal number of clusters Davies-Bouldin score}
\label{fig:Davies}
\end{figure}

\begin{figure}[H]
\hspace{-2cm}
\centering
\includegraphics[width=16cm]{scatter_research.png}
\caption{Research on SC grouped to 14 topics}
\href{https://github.com/QuantLet/CSC_Dapps}{\includegraphics[keepaspectratio,width=0.4cm]{media/qletlogo_tr.png}}
\label{fig:research_scatter}
\end{figure}


\textcolor{red}{
PLOT KEYWORDS WITHIN YEARS \\
ADJUST SIZES
}\\
\begin{figure}[H]
\hfill
\subfigure[Topic 1]{\includegraphics[width=5.3cm]{CSC/images/topics/Topic_0.png}}
\hfill
\subfigure[Topic 2]{\includegraphics[width=5cm]{CSC/images/topics/Topic_1.png}}
\hfill
\subfigure[Topic 3]{\includegraphics[width=4.9cm]{CSC/images/topics/Topic_2.png}}
\hfill
\subfigure[Topic 4]{\includegraphics[width=5.5cm]{CSC/images/topics/Topic_3.png}}
\hfill
\subfigure[Topic 5]{\includegraphics[width=4.9cm]{CSC/images/topics/Topic_4.png}}
\hfill
\subfigure[Topic 6]{\includegraphics[width=5cm]{CSC/images/topics/Topic_5.png}}
\hfill
\subfigure[Topic 7]{\includegraphics[width=5.4cm]{CSC/images/topics/Topic_6.png}}
\hfill
\subfigure[Topic 8]{\includegraphics[width=5cm]{CSC/images/topics/Topic_7.png}}
\hfill
\subfigure[Topic 9]{\includegraphics[width=4.7cm]{CSC/images/topics/Topic_8.png}}
\hfill
\href{https://github.com/QuantLet/CCID/tree/master/CCIDvolumeGAM}{\includegraphics[keepaspectratio,width=0.4cm]{media/qletlogo_tr.png}}
\caption{Top 10 the most important words per topic identified in the existing SC research (Part 1)}
\label{fig:topics_research_1}
\end{figure}

\begin{figure}[H]
\hfill
\subfigure[Topic 10]{\includegraphics[width=5.4cm]{CSC/images/topics/Topic_9.png}}
\hfill
\subfigure[Topic 11]{\includegraphics[width=4.8cm]{CSC/images/topics/Topic_10.png}}
\hfill
\subfigure[Topic 12]{\includegraphics[width=5.1cm]{CSC/images/topics/Topic_11.png}}
\hfill
\subfigure[Topic 13]{\includegraphics[width=5.5cm]{CSC/images/topics/Topic_12.png}}
\hfill
\subfigure[Topic 14]{\includegraphics[width=5.2cm]{CSC/images/topics/Topic_13.png}}
\hfill
\includegraphics[width=4cm]{CSC/images/topics/empty.png}
\hfill
\href{https://github.com/QuantLet/CCID/tree/master/CCIDvolumeGAM}{\includegraphics[keepaspectratio,width=0.4cm]{media/qletlogo_tr.png}}
\caption{Top 10 the most important words per topic identified in the existing SC research (Part 1)}
\label{fig:topics_research_2}
\end{figure}


 \textcolor[HTML]{FFBF00}{ssdXXXXXXXXXXXXXXsd}
 
 

Our research therefore reveals the tension between SC's and their implementation at the core of BC-related problems, that are not touched by individual research outlets as these primarily look at issues within their specific domain, like say the technological security of SC's or the legal handling of said. Yet, the system of this BC era is rapidly growing globally and is therefore increasingly complex and difficult to manage when only looking at individual aspects of the problem as a whole. Respectively, technological and regulatory responses to macro-level thrifts continue to only focus on the micro-level resulting in increasingly fragmented efforts to solve systemic BC issues with therefore limited effects. Contrasting against that background, we explicitly target the core understanding of the macro-structural and microtransactional functional aspects of the BC challenge outlined by SC's to achieve an assertive, comprehensive, and normatively unified basis.\\
 
 
 
 
 
 \vspace{8cm}
 
 


\textcolor{red}{COHERENCY JUMPING}\\
\textcolor{red}{RESEARCH QUESTIONS}\\


 \textcolor{red}{ technology, technocracy, and statistical finance}\\












%%%%%%%%%%%%NEXT%%%%%%%%%%%%%%






 
 
 

==> deprecated-tex/table_topics.tex <==
\begin{center}
 \begin{tabular}{||c c||} 
 \hline
 Topic & Amount of Research Papers \\ [0.5ex] 
 \hline\hline
 \textcolor[HTML]{286896}{Blockchain general} & 76 \\ 
 \hline
 \textcolor[HTML]{de762b}{Bitcoin/cryptocurrency research} & 95  \\
 \hline
 \textcolor[HTML]{338734}{Voting/payment} & 66  \\
 \hline
 \textcolor[HTML]{b93638}{Authorization/access} & 52  \\
 \hline
 \textcolor[HTML]{8766a8}{Ponzi/vulnerabilities (non-technical)} & 44  \\
 \hline
 \textcolor[HTML]{79514a}{Manufacturing} & 49  \\
 \hline
 \textcolor[HTML]{d179b4}{Oracle/cloud} & 77 \\
 \hline
 \textcolor[HTML]{6a6a6a}{Agriculture/food} & 105 \\
 \hline
 \textcolor[HTML]{9fa132}{Mining/validating} & 72 \\ 
 \hline
 \textcolor[HTML]{23a1af}{SC research papers} & 15  \\ 
 \hline
 \textcolor[HTML]{0a1064}{Healthcare/medical} & 26 \\
 \hline
 \textcolor[HTML]{7c39c3}{Attacks/vulnerabilities (technical)} & 97  \\
 \hline
 \textcolor[HTML]{e78379}{Auction/bidding} & 29\\
 \hline
 \textcolor[HTML]{429a68}{Energy prosumer} & 36 \\ [1ex] 
 \hline
\end{tabular}
\end{center}\label{Tab:Topics_amount}
